Adversarial and Reactive Traffic Entities for Behavior-Realistic Driving Simulation: A Review

Despite advancements in perception and planning for autonomous vehicles (AVs), validating their performance remains a significant challenge. The deployment of planning algorithms in real-world environments is often ineffective due to discrepancies between simulations and real traffic conditions. Evaluating AVs planning algorithms in simulation typically involves replaying driving logs from recorded real-world traffic. However, entities replayed from offline data are not reactive, lack the ability to respond to arbitrary AV behavior, and cannot behave in an adversarial manner to test certain properties of the driving policy. Therefore, simulation with realistic and potentially adversarial entities represents a critical task for AV planning software validation. In this work, we aim to review current research efforts in the field of traffic simulation, focusing on the application of advanced techniques for modeling realistic and adversarial behaviors of traffic entities. The objective of this work is to categorize existing approaches based on the proposed classes of traffic entity behavior and scenario behavior control. Moreover, we collect traffic datasets and examine existing traffic simulations with respect to their employed default traffic entities. Finally, we identify challenges and open questions that hold potential for future research.

==> content/00_frontmatter.tex <==
\title{Adversarial and Reactive Traffic Entities for Behavior-Realistic Simulation: A Review}

\author{\IEEEauthorblockN{Joshua Ransiek, Philipp Reis, Tobias Schürmann and Eric Sax}
\IEEEauthorblockA{\textit{FZI Research Center for Information Technology} \\
Karlsruhe, Germany \\
ransiek@fzi.de}
}

\maketitle
\thispagestyle{empty}
\pagestyle{empty}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
%In recent years, there have been notable advancements in perception and planning functions for \acp{AV}, yet the challenge of validating \acp{AV} performance remains largely unresolved. 
Despite advancements in perception and planning for \acp{AV}, validating their performance remains a significant challenge.
The deployment of planning algorithms in real-world environments is often ineffective due to discrepancies between simulations and real traffic conditions. 
Evaluating \acp{AV} planning algorithms in simulation typically involves replaying driving logs from recorded real-world traffic.
However, entities replayed from offline data are not reactive, lack the ability to respond to arbitrary \ac{AV} behavior, and cannot behave in an adversarial manner to test certain properties of the driving policy. 
Therefore, simulation with realistic and potentially adversarial entities represents a critical task for \ac{AV} planning software validation. 
In this work, we aim to review current research efforts in the field of traffic simulation, focusing on the application of advanced techniques for modeling realistic and adversarial behaviors of traffic entities.
The objective of this work is to categorize existing approaches based on the proposed classes of traffic entity behavior and scenario behavior control.  
Moreover, we collect traffic datasets and examine existing traffic simulations with respect to their employed default traffic entities.
\end{abstract}


==> content/05_evaluation_metrics.tex <==
\section{Evaluation Metrics}

Evaluation metrics are crucial in traffic simulation as they provide a quantitative measure of the simulated traffic agents to assess realism. 
These metrics are specifically designed to assess various aspects of the simulation and can be utilized to compare the simulated results with real-world data or other simulation models.
%Moreover, these metrics can be utilized as components of objective functions or regularization terms for learning-based agents.
Consistent with the perspective provided in \cite{montali_waymo_2024} and \cite{hu_solving_2024}, we define the following categories of metrics.

\subsection{Imitation Metrics}
Imitation metrics directly compare the performance of traffic agents to human demonstrations or other baselines to measure the scenario reconstruction ability. 
For instance, \cite{xu_bits_2023,vinitsky_nocturne_2022,gulino_waymax_2024} utilize \ac{ADE}, which calculates the average position differences between simulated and recorded agent trajectories. \cite{cornelisse_human-compatible_2024} extends this approach by incorporating the agent's goal, proposing goal-conditioned \ac{ADE}.
Additionally, the \ac{FDE} is employed to compare the final positions of simulated and recorded trajectories \cite{xu_bits_2023, vinitsky_nocturne_2022}. 
In \cite{cornelisse_human-compatible_2024}, the deviation of traffic agents' steering and acceleration actions from inferred human driving actions is used to compute the \ac{MASE} and \ac{MAAE}.
In contrast, imitation dataset metrics compare the driving profiles of simulated trajectories with those recorded in the dataset by generating histograms of key values such as velocity, acceleration, and jerk \cite{yan_learning_2023}. To compare these histograms, the Wasserstein distance is applied to measure the distance between the distributions \cite{xu_bits_2023}, or the Jensen–Shannon divergence is used to evaluate the similarity \cite{igl_symphony_2022}.

\subsection{Interaction Metrics}

Interaction metrics evaluate the interactions between traffic participants to assess safety and criticality. 
An intuitive approach to assess the safety of a scenario is by measuring the number or occurrence rate of collisions. 
\cite{igl_symphony_2022, xu_bits_2023, vinitsky_nocturne_2022, montali_waymo_2024, gulino_waymax_2024, cornelisse_human-compatible_2024} calculate the scenario collision rate (SCR) as the fraction of agents that fail in each scenario, where failure is defined as an agent colliding with any other agent.
A collision is defined as an event that occurs when the bounding boxes of two agents overlap.
Furthermore, \cite{xu_bits_2023, sun_intersim_2022} classify agent collisions according to their type, including rear, front, and side collisions, noting that each agent can have multiple types of collisions within a single scenario.
\cite{montali_waymo_2024} calculates the distance to the nearest object at each time step throughout the scenario.
To measure the behavioral safety of traffic participants and analyze traffic conflicts, criticality metrics have been proposed, including the well-known \ac{TTC} \cite{minderhoud_extended_2001} employed in \cite{montali_waymo_2024}. 
For a comprehensive review of scenario criticality measures and agent interactions, see \cite{westhofen_criticality_2023}.  
\cite{shalev-shwartz_formal_2017} proposes a mathematical model for safety assurance, called \ac{RSS}.
\cite{chandra_cmetric_2020} classifies driver behaviors using centrality functions.

\subsection{Map Metrics}

Map metrics facilitate the comparison of agent behavior to drivable/walkable spaces, traffic rules, and desired map positions for traffic agents. 
An agent that controls a vehicle and leaves the drivable space is considered off-road. \cite{xu_bits_2023, gulino_waymax_2024, montali_waymo_2024, cornelisse_human-compatible_2024} calculate the off-road rate as the fraction of agents that fail in each scenario, where failure is defined as an agent driving off the road.
Additionally, \cite{montali_waymo_2024} calculates the distance to the road edge at each time step throughout the scenario.
Traffic rule compliance is assessed by checking adherence to traffic light signals \cite{suo_trafficsim_2021}, stop signs \cite{zhong_guided_2023} and speed limits \cite{zhong_guided_2023}.
\cite{gulino_waymax_2024} examines the phenomenon of wrong-way driving. 
The assessment of goal-reaching behavior involves calculating the goal rate as the number of vehicles that achieve their goal position within a scenario's simulation \cite{vinitsky_nocturne_2022, cornelisse_human-compatible_2024}. 
In this context, \cite{sun_intersim_2022} defines progress as the total traveled distance of all simulated agents divided by the number of simulated agents, providing a metric to measure the level of goal achievement. 
To measure the diversity across simulation rollouts, \cite{xu_bits_2023} calculates the coverage metric, which assesses the map area covered by multiple simulation trials with the same initial conditions. Additionally, the diversity metric computes the Wasserstein distances among the density profiles of map coverage achieved in different simulation trials.

\subsection{Kinematic Metrics}

Kinematic metrics assess the feasibility of agents' actions, such as steering and acceleration \cite{gulino_waymax_2024}, or, additionally, velocity, angular velocity, and angular acceleration \cite{montali_waymo_2024}, by evaluating them against predefined value ranges. 

\subsection{Language Metrics}



==> content/08_supplemental_material.tex <==
\section{Comparison of Traffic Simulators}

\newpage
\section{Comparison of Trajectory Datasets}

\begin{table}[h!]
    \footnotesize
    \centering
    \caption{Comparison of recent trajectory datasets for road vehicles inspired by \cite{caesar_nuplan_2021, gressenbuch_mona_2022}. \textit{Record time}: Total duration of recorded trajectory data. \textit{Scenes}: Number of distinct locations. \textit{Sampling Frequency}: Frequency of trajectory positions. \textit{Sensor Data}: Availability of sensor data. \textit{Type}: Type of dataset, which can be either prediction ("Pred") or planning ("Plan").} 
    \begin{tabular}{lccccc}
        \toprule
        Dataset & \makecell{Record\\time} & \makecell{Scenes} & \makecell{Sampling \\ frequency} & \makecell{Sensor \\ data} & Type \\
        \midrule 

        CommonRoad \cite{althoff_commonroad_2017} & - & 39799 & 10 Hz & & Plan \\

        highD \cite{krajewski_highd_2018} & 16.5 h & 6 & 25 Hz & & Pred\\

        Argoverse 1 \cite{chang_argoverse_2019} & 320 h & 323,557 & 10 Hz & & Pred\\
        
        Interaction \cite{zhan_interaction_2019} & 10 h & 11 & 10 Hz & & Pred\\

        inD \cite{bock_ind_2020} & 10 h & 4 & 10 Hz & & Pred\\

        openDD \cite{breuer_opendd_2020}&  62 h & 7 & 10 Hz & & Pred\\

        nuPredict \cite{caesar_nuscenes_2020} \tablefootnote[1]{Human-labeled scenes from the nuScenes datase} & 5.5 h & 850 & 2 Hz & $\surd$ & Pred\\

        Waymo \cite{sun_scalability_2020} & 570 h & 103,354 & 10 Hz & &  Pred\\

        Lyft Level 5 \cite{houston_one_2021} & 1118 h & 170,000 & 10 Hz & & Pred\\

        Shifts \cite{malinin_shifts_2021} & 1667 h & - & 5 Hz & & Pred \\

        MONA \cite{gressenbuch_mona_2022} & 130 h & 3 & 5 Hz & & Pred \\ 

        Argoverse 2 \cite{wilson_argoverse_2023} & 763 h & 250,000 & 10 Hz& & Pred\\

        nuPlan \cite{caesar_nuplan_2021, karnchanachari_towards_2024} & 1282 h & - & 10 Hz & $\surd$ & Plan\\
        \bottomrule
    \end{tabular}
    \label{tab:datasets}
\end{table}

%\section{Definition of Evaluation Metrics} \label{sec:metrics_definitions}
%
%\subsection{Non-learned Evaluation Metrics}
%
%\textbf{Scene Average Displacement Error (SADE)}: 
%\begin{equation}
%\text{sADE} = \frac{1}{K_{te} N_I T} \sum_{k=1}^{K_{te}} \left[\sum_{i \in I} \sum_{t=1}^{T} \delta\left(s^{i}_{k,t}, s'^{i}_{k,t}\right)\right]
%\end{equation}
%where $I$ is the set of indices of the interactive agents, $s'^{i}_{k,t}$ and $s^{i}_{k,t}$ are the states of the $i^{th}$ interactive agents in the $k^{th}$ simulated and reference trajectories, respectively, and $\delta$ is a Euclidean distance function. \cite{igl_symphony_2022}

%\textbf{Minimum Scene Average Displacement Error (minSADE)}: 
%\begin{equation}
%\text{minSADE} = \frac{1}{K_{te} N_I T} \sum_{k=1}^{K_{te}} \min_{r' \in R_k} \left[ \sum_{i \in I} \sum_{t=1}^{T} \delta\left(s^{i}_{k,t}, s'^{i}_{k,t}\right) \right],
%\end{equation}
%when $m = 1$, minSADE reduces to SADE; when $m > 1$, minimising minSADE requires populating Rk with diverse but realistic trajectories. \cite{igl_symphony_2022}

%\textbf{Coverage (cov) and diversity (div)}: 
%\begin{equation}
%    \text{Diversity} = \frac{2}{n(n-1)} \sum_{i=1}^{n-1} \sum_{j=i+1}^{n} \text{Wass}(\rho_i,\rho_j),
%\end{equation}
%where $\text{Wass}(\cdot,\cdot)$ is the Wasserstein distance and $\rho_i$ is the density profile for the $i$-th trail.

%\subsection{Learned Evaluation Metrics}
